Inferences from surface brightness fluctuations of Zwicky 3146 via the Sunyaev-Zeldovich effect and X-ray observations

The galaxy cluster Zwicky 3146 is a sloshing cool core cluster at $z{=}0.291$ that in SZ imaging does not appear to exhibit significant pressure substructure in the intracluster medium (ICM). We perform a surface brightness fluctuation analysis via Fourier amplitude spectra on SZ (MUSTANG-2) and X-ray (XMM-Newton) images of this cluster. These surface brightness fluctuations can be deprojected to infer pressure and density fluctuations from the SZ and X-ray data, respectively. In the central region (Ring 1, $r < 100^{\prime\prime} = 440$ kpc, in our analysis) we find fluctuation spectra that suggest injection scales around 200 kpc ($\sim 140$ kpc from pressure fluctuations and $\sim 250$ kpc from density fluctuations). When comparing the pressure and density fluctuations in the central region, we observe a change in the effective thermodynamic state from large to small scales, from isobaric (likely due to the slow sloshing) to adiabatic (due to more vigorous motions). By leveraging scalings from hydrodynamical simulations, we find an average 3D Mach number $\approx0.5$. We further compare our results to other studies of Zwicky 3146 and, more broadly, to other studies of fluctuations in other clusters.

==> MachTable2Rings.tex <==
\begin{table}[!h]
    \begin{center}
    \begin{tabular}{c c| c c | c c}
        \hline
          & & $\mathcal{M}_{\text{3D}}$ & $d \ln P_{\text{th}} / d \ln r$ & $d \ln \mathcal{M}_{\text{3D}} / d \ln r$ & $-b_{\mathcal{M}}$ \\
          \hline
        \multirow{2}{*}{Ring 1} & X-ray & $1.12 \pm 0.01$ & \multirow{2}{*}{$-1.32 \pm 0.09$} & \multirow{2}{*}{$-0.002 \pm 0.30$} & $0.41 \pm 0.10$ \\
                                & SZ    & $1.42 \pm 0.40$ & & & $0.53 \pm 0.17$ \\
                                \hline
        Ring 2 & X-ray & $1.19 \pm 0.37$ & $-1.78 \pm 0.29$   & $0.002 \pm 0.30$ & $0.41 \pm 0.19$ \\
                                \hline
        \end{tabular}
        \end{center}
    \caption{Deduced values from amplitude spectra following methods employed in \citet{khatri2016}.}
    \label{tbl:b_from_ps}
\end{table}


==> MachTable3Rings.tex <==
\begin{table}[!h]
    \begin{center}
    \begin{tabular}{c c| c c | c c | c c}
        \hline
          & & $\mathcal{M}_{\text{3D}}$ & $d \ln P_{\text{th}} / d \ln r$ & $d \ln \mathcal{M}_{\text{3D}} / d \ln r$ & $-b_{\mathcal{M}}$ & $d \ln \mathcal{M}_{\text{3D}} / d \ln r$ & $-b_{\mathcal{M}}$  \\
          \hline
        \multirow{2}{*}{Ring 1} & X-ray & $1.12 \pm 0.01$ & \multirow{2}{*}{$-1.32 \pm 0.09$} & \multirow{2}{*}{$-1.02 \pm 0.13$} & $0.006 \pm 0.272$ & \multirow{2}{*}{$0.71 \pm 0.35$} & $0.035 \pm 0.306$ \\
                                & SZ    & $1.42 \pm 0.40$ & & & $0.01 \pm 0.43$ & & $0.055 \pm 0.470$ \\
                                \hline
        \multirow{2}{*}{Ring 2} & X-ray & $1.29 \pm 0.83$ & \multirow{2}{*}{$-1.78 \pm 0.29$} & \multirow{2}{*}{$3.06 \pm 1.78$} & $-0.02 \pm 3.86$  & \multirow{2}{*}{$0.71 \pm 0.35$} & $0.046 \pm 0.400$ \\
                                & SZ    & $4.52 \pm 4.05$ & & & $-0.36 \pm 83$ & & $0.37 \pm 2.15$ \\
                                \hline
        Ring 3 & X-ray & $6.92 \pm 5.30$ & $-6.30 \pm 5.12$ & $2.92 \pm 2.24$ & $0.95 \pm 0.13$ & $0.71 \pm 0.35$ & $0.58 \pm 2.23$ \\
        \hline
        \end{tabular}
        \end{center}
    \caption{Deduced values from amplitude spectra following methods employed in \citet{khatri2016}.}
    \label{tbl:b_from_ps}
\end{table}


==> hydrostatic_bias.tex <==
\subsection{Hydrostatic mass bias}

We have multiple ways of indirectly estimating the non-thermal pressure support, specifically as a single quantity termed the hydrostatic bias, 
\begin{equation}
    b = 1 - M_{\text{HSE}}/M_{\text{tot}}.
    \label{eqn:mass_bias}
\end{equation}
The simplest estimate can come from taking the total mass, $M_{\text{tot}}$ to be equal to the weak lensing mass, $M_{\text{WL}}$\footnote{This is not to say that weak lensing mass estimates are without their own systematic uncertainties or biases.}. For this system, \citet{romero2020} used the weak lensing mass from \citet{klein2019} to find $b = 0.07 \pm 0.29$ with $M_{\text{HSE}} = 7.69_{-1.98}^{+2.19} \times 10^{14} M_{\odot}$ and $M_{\text{WL}} = 8.28_{-1.20}^{+1.19} \times 10^{14} M_{\odot}$. An updated profile fit yields  $M_{\text{HSE}} = 6.93_{-2.95}^{+2.82} \times 10^{14}$ with a corresponding bias of $b = 0.16 \pm 0.37$, where we adopt the same mean molecular mass, $\mu = 0.61$ as previously, i.e. in \citet{romero2020}.

Another avenue to quantifying the hydrostatic bias can be to assume a universal value of the gas mass fraction to obtain a total mass:
\begin{equation}
    f_{\text{gas}}(r) = \frac{M_{\text{gas}}(<r)}{M_{\text{tot}}(<r)}, 
\end{equation}
where values of $f_{\text{gas}}(R_{500})$ are reported in \citet{ghirardini2018,mantz2016b}, both of which find $f_{\text{gas}}(R_{500}) = 0.125$. With this value, we find $M_{\text{tot}} = 8.22 \pm 0.37 \times 10^{14} M_{\odot}$, which is quite close to the weak lensing mass estimate from \citet{klein2019}. By extension, the hydrostatic bias inferred in this manner is $b = 0.16 \pm 0.35$.

We can also infer non-thermal pressure support from our amplitude spectra presented in Section~\ref{sec:results}, where we particular make the assumption that the non-thermal pressure support comes from (quasi) turbulent gas motions. A simple approximation from \citet{Gaspari2013_PS} gives us:
\begin{equation}
    \mathcal{M}_{\text{3D}} \approx 4 A_{\rho}(k_{\text{peak}}) \approx 2.4 A_{P}(k_{\text{peak}})
\end{equation}

%\MG{We cannot use the peak for an inverted spectrum (and unresolved injection), please use only the first 2-3 modes for such conversion}
%Keeping with the bias as defined in Equation~\ref{eqn:mass_bias},

\citet{khatri2016} provide a relation between the hydrostatic bias and $\mathcal{M}_{\text{3D}}$ (and attach a corresponding subscript to denote the method of calculation, $b_{\mathcal{M}}$): %\MG{there should be a minus in front, added}:
\begin{equation}
    b_{\mathcal{M}} = \frac{-\gamma \mathcal{M}_{\text{3D}}^2}{3} \frac{ d \ln P_{\text{NT}}}{d \ln P_{\text{th}}} \left( 1 +  \frac{\gamma \mathcal{M}_{\text{3D}}^2}{3}\frac{ d \ln P_{\text{NT}}}{d \ln P_{\text{th}}} \right)^{-1},
    \label{eqn:mach_bias}
\end{equation}
where $\gamma$ is the adiabatic index, taken to be 5/3 for the ICM. NB that as defined in \citet{khatri2016} $b_{\mathcal{M}} \equiv M_x / M_{\text{tot}} - 1 = -b$. Following the recasting performed in \citet{khatri2016}, we find:
\begin{equation}
    \frac{ d \ln P_{\text{NT}}}{d \ln P_{\text{th}}} = \frac{ d \ln P_{\text{NT}} / d \ln r}{d \ln P_{\text{th}} / d \ln r} = 1 + 2 \frac{ d \ln \mathcal{M}_{\text{3D}} / d \ln r}{d \ln P_{\text{th}} / d \ln r}.
\end{equation}

\input{MachTable2Rings.tex}

The derivation of Equation~\ref{eqn:mach_bias} implies that quantities on the right hand side should be computed at the relevant radius; e.g. if we are interested in $b_{\mathcal{M}}(R_{500})$, then we should compute the respective values on the right hand side at $R_{500}$.
%where the difficulty largely comes from calculating $d \ln \mathcal{M}_{\text{3D}} / d \ln r$ at the relevant radii

%As we do not have a reliable amplitude spectrum for Ring 3, we choose instead to find what Mach number in Ring 3 would produce $b = 0.16 = -b_{\mathcal{M}}(R_{500})$. Rather than compute $d \ln \mathcal{M}_{\text{3D}} / d \ln r$ between rings, we start with a single slope calculated from Rings 1 and 2. Once we derive an initial value for $\mathcal{M}(r)$ in Ring 3 we fit a second order polynomial to $\mathcal{M}(r)$ in linear space, from which we can calculate $d \ln \mathcal{M}_{\text{3D}} / d \ln r$ for each ring assuming effective radii of $50^{\prime\prime}$, $150^{\prime\prime}$, and $250^{\prime\prime}$ for Rings 1, 2, and 3, respectively. We iterate this process until convergence wherein for Ring 3 we find that $\mathcal{M}_{\text{3D}} = 0.71$ will satisfy $-b_{\mathcal{M}}(R_{500}) = 0.16$. 

\textcolor{red}{The below discussion has to change -- our results have larger Mach numbers now.}

While we don't have a good means of comparing hydrostatic bias values in the inner rings, we can compare our derived $\mathcal{M}_{\text{3D}}$ value to $\mathcal{M}_{\text{1D}}$ values found in \citet{hofmann2016}, who studied fluctuations in 33 X-ray bright clusters. Specifically, in Zwicky 3146 they found a one-dimensional Mach number ($\mathcal{M}_{\text{1D}}$) of $\sim0.26$. Given that $\mathcal{M}_{\text{3D}}  = \sqrt{3} ~ \mathcal{M}_{\text{1D}}$, this would correspond to $\mathcal{M}_{\text{3D}}  = 0.45$. Their study adopted an analysis of the variation of deprojected bins in real-space (i.e. not Fourier space as in this work) and made use of \textit{Chandra} data which covered out to roughly $R_{500}/3$ for Zwicky 3146 (this is about average in their sample of 33 clusters).
Thus the appropriate comparison should be with Ring 1, where we recover lower $\mathcal{M}_{\text{3D}}$ values (0.19 from X-ray and 0.18 from SZ), while we find close agreement with our Ring 2 value from X-ray (0.44). Given the substantially different analysis methods, a thorough comparison is beyond the scope of this discussion. 

Notwithstanding the differences in approaches, \citet{hofmann2016} find most clusters have $\mathcal{M}_{\text{3D}}$ between $0.2$ and $0.4$ for their sample. Their values, along with our values here are thus broadly in agreement with each other, as well as with high resolution hydrodynamical simulations which find $\mathcal{M}_{\text{3D}} < 0.5$ \citep[e.g.][]{Gaspari2014_PS}.

%We should also consider that the Mach number derived for a given cluster in \citet{hofmann2016} is taken as either the pressure fractional spread or entropy fractional spread, whichever is greater. For Zwicky 3146, their average fractional spread of thermodynamic quantities are as follows: $\left| \delta P / P \right| = 0.004_{-0.004}^{+.023}$, $\left| \delta K / K \right| = 0.259_{-0.025}^{+.022}$, $\left| \delta T / T \right| = 0.109_{-0.019}^{+.019}$, and $\left| \delta n / n \right| = 0.159_{-0.013}^{+.009}$. 
%\MG{Please compare/mention the Mach numbers 3D of Ring 1-2 with the values found in Hofmann+16, Figure 10; in their larger sample 3D Mach numbers are in the range 0.2-0.4, as we find here, so good to discuss/emphasize this here.
%Also worth to add that this is consistent with high-resolution hydrodynamical simulations of galaxy clusters in a more relaxed state, i.e., having Mach $< 0.5$ (\citealt{Gaspari2014_PS})}.


\subsection{A comment on uncertainties}

We note that our hydrostatic mass biases when using our estimate of $M_{\text{HSE}}$ have large uncertainties predominantly because of the large uncertainties on $M_{\text{HSE}}$ itself. This can, of course, be (artificially) remedied by assuming some profile, such as a gNFW profile as noted in \citet{romero2020}. By extension, $d \ln P_{\text{th}} / d \ln r$ will see a significant reduction in uncertainty in Ring 3 if assuming a parametric profile. 

However, assuming a parametric profile for our SZ data will not improve the inferred amplitude spectra (much as we still encounter difficulties with X-ray data while assuming a double beta profile). An inherit difficulty with SZ and X-ray fractional fluctuation measurements is the effective increase in noise towards larger radii due to the division of smaller values of their respective surface brightness profiles. While the SZ surface brightness profile will decrease less rapidly relative to an X-ray surface brightness profile, the SZ map has decreasing sensitivity towards larger radii due to the instrument's instantaneous FOV and scanning strategy. The current observing strategy is adopted because it is among the most efficient in terms of telescope time and sensitivities achieved. This leaves an increase of FOV as a highly desirable improvement to better probe the outskirts of galaxy clusters with high resolution SZ measurements. 
%Given that the relation between $b_{\mathcal{M}}$ and $\mathcal{M}_{\text{3D}}$ depends also on $d \ln \mathcal{M}_{\text{3D}} / d \ln r$, we iteratively = -0.18 \pm 0.20$.


==> ps-products-without-kpeak.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{c c| c c c}
          & & $\alpha_k$ & $A_{\text{3D}}(k_{\text{peak}})$ & $\sigma^2$ \\
          \hline
        \multirow{2}{*}{Ring 1} & $\delta \rho/\rho$ & $2.5 \pm 0.1$ & $0.33 \pm 0.01$ & 0.15 \\
                                & $\delta P/P$    & $0.6 \pm 0.9$ & $0.57 \pm 0.17$ & 0.44 \\
                                \hline
         Ring 2 & $\delta \rho/\rho$ & $2.3 \pm 1.6$ & $0.27 \pm 0.09$ & 0.21 \\
                                %& SZ    & $0.6 \pm 2.2$ & [$0.93 \pm 0.76$] & [0.018 arcsec$^{-1}$] \\
                                \hline
       Ring 3 & $\delta \rho/\rho$ & $1.7 \pm 1.0$ & $1.68 \pm 0.53$ & 4.51 \\
                                \hline
        %Ring 3 & X-ray & $0.7 \pm 0.4$ & $0.28 \pm 0.03$ \\
        %                        \hline
    \end{tabular}
    \caption{Inferred spectral indices (logarithmic slope) and peaks of the amplitude spectra. The spectral indices assume a single power law across our sampled range with the exception of points at $k=0.01$ arcsec$^{-1}$ (we omit points at $k=0.01$ arcsec$^{-1}$). The peaks of amplitude spectra are taken with a signal-to-noise cut of 3.}
    \label{tbl:ps_products}
\end{table}

